Linear Cross-document Event Coreference Resolution with X-AMR

Event Coreference Resolution (ECR) as a pairwise mention classification task is expensive both for automated systems and manual annotations. The task's quadratic difficulty is exacerbated when using Large Language Models (LLMs), making prompt engineering for ECR prohibitively costly. In this work, we propose a graphical representation of events, X-AMR, anchored around individual mentions using a \textbf{cross}-document version of \textbf{A}bstract \textbf{M}eaning \textbf{R}epresentation. We then linearize the ECR with a novel multi-hop coreference algorithm over the event graphs. The event graphs simplify ECR, making it a) LLM cost-effective, b) compositional and interpretable, and c) easily annotated. For a fair assessment, we first enrich an existing ECR benchmark dataset with these event graphs using an annotator-friendly tool we introduce. Then, we employ GPT-4, the newest LLM by OpenAI, for these annotations. Finally, using the ECR algorithm, we assess GPT-4 against humans and analyze its limitations. Through this research, we aim to advance the state-of-the-art for efficient ECR and shed light on the potential shortcomings of current LLMs at this task. Code and annotations: \url{https://github.com/ahmeshaf/gpt_coref}

==> figures/evt-ids.tex <==

\begin{table}[h]
    \centering
    \resizebox{\textwidth/2 - 10pt}{!}{
    \begin{tabular}{|c|l|}
    \hline
    \multicolumn{2}{|c|}{\eid} \\
    \hline
    a & $\langle \HP\pbSyns\EYP \rangle$ \\
    \hline
    b & $\langle \HP, \pbSyns(\mathrm{purchase.01}), \EYP \rangle$ \\
    \hline
    c & $\langle\HP, \pbSyns(\mathrm{state.01}), \EYP\rangle$ \\
    \hline
    d & \makecell[l]{$\langle \HP, \pbSyns(\mathrm{announce.01}), \HP, \pbSyns(\mathrm{acqure.01}),\EYP \rangle$ \\ 
        $\langle \HP, \pbSyns(\mathrm{announce.01}),\HP, \pbSyns(\mathrm{sign.02}),$ \\
        $\hspace{43mm}\HP, \pbSyns(\mathrm{acquire.01}), \EYP\rangle$} \\
    \hline
    \end{tabular}}
  \caption[Event Identifiers]{
	Event Identifiers for examples in Figure \ref{fig:evt-coref} }
\label{tab:evt-ids}
\end{table}

==> test_results.tex <==
\begin{table}[t]
% \renewcommand{\arraystretch}{1.5}
\centering
\small
\resizebox{\textwidth/2 - 8.5pt}{!}{
    \begin{tabular}{@{}c|lccccc@{}}
        \toprule
        % \multicolumn{1}{c}{~}&&&
        % \multicolumn{4}{c}{All Events} \\
        % \cmidrule{4-7}
       \multicolumn{1}{c}{~}& Method && R$_{avg}$ & P$_{avg}$ & \conll & LEA \\ 
        \midrule
        \multicolumn{1}{c}{~}&\LEM && 70.6 & 73.2 & 71.6 & 56.0 \\
 \hline

  \multirow{6}{*}{\rotatebox{90}{\annone}}
  &\RSHum 
 && 79.4 & 70.0 & 73.4 & 58.0
\\
&\eidNH
 && 60.6 & \textbf{88.3} & 71.5 & 59.4
\\
& \eidNH~\OR~\eidLTH
 && 68.8 & 87.4 & \textbf{76.3} & \textbf{64.8}
\\  
  &\RSVN
 && \textbf{91.3} & 39.8 & 45.9 & 28.8
\\
&\eidHVN
 && 66.8 & 76.7 & 70.5 & 56.0
\\
&\eidHVN~\OR~\eidLTHVN
 && 77.0 & 64.8 & 68.8 & 52.7
\\
%   &$\RSHum_\PBSynHum$
%  && 89.6 & 49.6 & 56.5 & 41.1
% \\
% &$\RSHum_\PBSynHum + \eid$
%  && 70.2 & 81.1 & 74.8 & 61.7
% \\
% &$\RSHum_\PBSynHum + \eidLT$
%  && 82.0 & 64.5 & 70.2 & 53.2
% \\

\hline
\multirow{3}{*}{\rotatebox{90}{GPT}}& \RSGPT
&& 68.0 & 65.8 & \textbf{67.6} & \textbf{49.8} 
\\
% &$\RSGPT + \eid$
% && 42.6 & \textbf{84.9} & 58.8 & 46.8 
% \\
% &$\RSGPT + \eidLT$
% && 52.8 & 77.1 & 64.2 & 48.8 \\
% &$\RSGPT_\PBSynVN$
%  && \textbf{81.5} & 42.4 & 49.8 & 30.6
% \\
&\eidLEM
 && 42.8 &\textbf{ 91.2} & 60.1 & 49.6
\\
&\eidLEM~\OR~\eidLTLEM
 && 54.2 & 85.4 & 67.2 & 54.0
\\
\hline
\multicolumn{1}{c}{~}&SotA && &  & \textbf{87.4} & \textbf{79.4} \\
 \hline
\bottomrule

% &$\RSGPT_\PBSynHum$
%  && 74.7 & 54.4 & 60.7 & 42.1
% \\
% &$\RSGPT_{\PBSynHum} + \eid$
%  && 47.6 & 80.2 & 61.2 & 46.9
% \\
% &$\RSGPT_\PBSynHum + \eidLT$
%  && 59.4 & 67.1 & 63.2 & 45.1
% \\

        % \midrule
        % RS-only & 69.9 & 60.2 & 56.0 & 62.0 \\ \hline
        % EID-only & 62.8 & 73.2 & 67.9 & 68.0 \\ \hline
        % EID+VN & 63.9 & 72.9 & 65.9 & 67.6 \\  \hline
    \end{tabular}
    }
  % \vspace*{-2mm}
  \caption[\ecb~Results]{
	\ecb~Results comparing the annotators and GPT-4. }
\label{tab:ecb_res_ann}
\end{table}


==> verbs.tex <==
\begin{minipage}[b]{0.35\columnwidth}
% \hspace{-10mm}
\begin{verbatim}
agree.01
  Arg0: HP 
  Arg1: acquire.01
    Arg1: EYP
\end{verbatim}
\end{minipage}

\hspace{0.5cm}

\begin{minipage}[b]{0.50\columnwidth}
\begin{verbatim}
(a /agree.01
    :Arg0 (h /HP) 
    :Arg1: (a2 /acquire.01
        :Arg1 (h)
        :Arg4 (e /EYP) ))
\end{verbatim}
\end{minipage}
